Influence of Disorder and Anharmonic Fluctuations on the Dynamical Rashba Effect in Purely Inorganic Lead-Halide Perovskites

Doping organic metal-halide perovskites with cesium could be the best solution to stabilize highly-efficient perovskite solar cells. The understanding of the respective roles of the organic molecule, on one hand, and the inorganic lattice, on the other, is thus crucial in order to be able to optimize the physical properties of the mixed-cation structures. In particular, the study of the recombination mechanisms is thought to be one of the key challenges towards full comprehension of their working principles. Using molecular dynamics and frozen phonons, we evidence sub-picosecond anharmonic fluctuations in the fully inorganic $CsPbI_3$ perovskite. We reveal the effect of these fluctuations, combined with spin-orbit coupling, on the electronic band structure, evidencing a dynamical Rashba effect. Our study show that under certain conditions space disorder can quench the Rashba effect. As for time disorder, we evidence a dynamical Rashba effect which is similar to what was found for $MAPbI_3$ and which is still sizable despite temperature disorder, the large investigated supercell, and the absence of the organic cations' motion. We show that the spin texture associated to the Rashba splitting cannot be deemed responsible for a consistent reduction of recombination rates, although the spin mismatch between valence and conduction band increases with the ferroelectric distortion causing the Rashba splitting.

==> makefile <==
TEX=/usr/bin/pdflatex
PLAINLATEX=latex
TAR=tar
ZIP=/usr/bin/zip
AWK=awk
MAIN=achemso_new
SI=SI
GREP=grep
OTHER=SI.tex SI.pdf ${MAIN}.bbl
BIB=sample_clean.bib
#SOURCES=${MAIN}.tex  introall.tex computational_details.tex results.tex discussion.tex ${BIB} 
SOURCES=${MAIN}.tex  ${BIB} ${SI}.tex
STYLES=TEXINPUTS/achemso.zip
TEXT=${SOURCES}
FIGS=`${GREP} includegra ${TEXT}|${AWK} '$$1!~"%" {gsub("{"," ");gsub("}"," ");for (i=1;i<=NF;i++){if ($$(i)~"eps" || $$(i)~"png") {figname=$$(i)}};printf "%s ", figname}END{printf "\n" }' `

pdf: 
	${TEX} ${MAIN}.tex; bibtex ${MAIN}.aux ; ${TEX} ${MAIN}.tex ; ${TEX} ${MAIN}.tex
SIpdf: 
	${TEX} ${SI}.tex ; ${TEX} ${SI}.tex
#; bibtex ${SI}.aux ; ${TEX} ${SI}.tex ; ${TEX} ${SI}.tex

count:${SOURCES}
	@awk '$$1!~"^%" {print $$0}' ${SOURCES} |wc
textcount:${TEXT}
	@awk '$$1!~"^%" {print $$0}' ${TEXT} |wc
clean: 
	/bin/rm *.log *.toc *.aux *.dvi *.blg *.bbl *.spl ${MAIN}.pdf ${SI}.pdf
tar: 
	${TAR} zhcvf RashbaPaper`/usr/bin/date  -u +%d%b%Y`.tar.gz ${SOURCES} ${FIGS} ${STYLES} makefile ${MAIN}.pdf ${OTHER}
zip:	
	${ZIP} RashbaPaper`/usr/bin/date  -u +%d%b%Y`.zip ${SOURCES} ${FIGS} ${STYLES} makefile ${MAIN}.pdf ${OTHER}

